Strengthening Order Preserving Encryption with Differential Privacy

Ciphertexts of an order-preserving encryption (OPE) scheme preserve the order of their corresponding plaintexts. However, OPEs are vulnerable to inference attacks that exploit this preserved order. At another end, differential privacy has become the de-facto standard for achieving data privacy. One of the most attractive properties of DP is that any post-processing (inferential) computation performed on the noisy output of a DP algorithm does not degrade its privacy guarantee. In this paper, we propose a novel differentially private order preserving encryption scheme, OP$\epsilon$. Under OP$\epsilon$, the leakage of order from the ciphertexts is differentially private. As a result, in the least, OP$\epsilon$ ensures a formal guarantee (specifically, a relaxed DP guarantee) even in the face of inference attacks. To the best of our knowledge, this is the first work to combine DP with a property-preserving encryption scheme. We demonstrate OP$\epsilon$'s practical utility in answering range queries via extensive empirical evaluation on four real-world datasets. For instance, OP$\epsilon$ misses only around $4$ in every $10K$ correct records on average for a dataset of size $\sim732K$ with an attribute of domain size $\sim18K$ and $\epsilon= 1$.

==> formal_model.tex <==
\section{\nam and Inference Attacks} \label{sec:attack} 
 \begin{figure}[ht]
      \includegraphics[width=\linewidth]{ppt_diag.pdf}\vspace{-0.3cm}
        \caption{Relationships between \ddp, \cdp and \indfaocpa guarantees.} \label{fig:relation}\vspace{-0.5cm}
    \end{figure}
    %\vspace{-0.2cm}
   In this section, we discuss the implications of \nam's security guarantee  in the face of inference attacks. \par 
 Recall that intuitively, the \indfaocpae~ guarantee of a \nam schemes bolsters the cryptographic guarantee of a \OPE scheme (\indfaocpa) with an additional layer of a relaxed \DP guarantee. For the rest of the discussion, we focus on the worst case scenario where the \OPE scheme provides no protection at all and study what formal guarantee we can achieve from just the (relaxed) \DP guarantee. \par 
As discussed in Sec. \ref{sec:background:DP}, our proposed distance-based relaxation of \DP comes in two flavors -- local (\ddp, Def. \ref{def:ddp})  and central (\cdp, Def. \ref{def:cdp}). Intuitively, \ddp is a guarantee for each individual data point while \cdp is a guarantee for a dataset.  As a refresher, Fig. \ref{fig:relation} showcases the relationships between them. The most salient points are: \begin{itemize}\item \ddp is a stronger guarantee than \cdp -- $\epsilon$-\ddp implies $\epsilon$-\cdp. Thus, owing to the \ddp guarantee of the underlying \name-primitive, \nam trivially satisfies both \ddp (Lemma \ref{lem:ddp}) and \cdp (Lemma \ref{lem:cdp} App. \ref{app:thm:main}) guarantees. \item The \cdp guarantee can be amplified via shuffling (Thm. \ref{thm:amplify:1} App. \ref{app:amplify}, Thm. \ref{thm:amplify}). \end{itemize}
 Now, we show how to interpret the protection provided by both these guarantees via an indistinguishability game, as is traditional for cryptographic security definitions. Let the input be drawn from a discrete domain of size $N$, i.e., $|\mathcal{X}|=N$. The dataset indistinguishability game, $(\alpha,\beta)-\textsf{DI}$, is characterized by two parameters -- precision parameter $\alpha \in [\frac{1}{N},1]$ and recovery rate $\beta \in [\frac{1}{n},n]$ where $n$ is the dataset size.   For a given dataset $X$, an adversary has to distinguish among $X$ and  a set of datasets $Q(X)$ such that  any  pair of datasets $(X,X')$, where $X' \in Q(X)$ and $X'=\{x'_1,\cdots,x'_n\}$, \begin{enumerate}\item differ in at most $\beta n$ data points corresponding to the indices $R=\{j|j \in [n]\}, |R|=\lceil\beta n\rceil$, i.e., \begin{gather}x'_j=x_j \thinspace\forall j \in [n], j \not\in R \label{eq:1}\end{gather} \item  the corresponding values for the indices in $R$ differ at most by $\lceil\alpha N\rceil$, i.e., \begin{gather} |x_{j}-x'_{j}|\leq \lceil\alpha N\rceil, \thinspace \forall j \in R\label{eq:2}\end{gather}\end{enumerate} 
 
 For example, consider $\mathcal{X}=[1-10], N=10, n=5, \alpha=1/5$, $\beta=1/5, X=\{2,6,7,8,9\}$ and $Q=\{2,4\}$. This means $X$ and that the datasets in $Q(X)$ can differ only in $\lceil\beta n\rceil=2$ points corresponding to the indices $2$ and $4$, and their values should be within distance $\lceil\alpha N\rceil=1$ from each other. Thus, the adversary has to distinguish among $X$ and the following $8$ datasets $Q(X)=\Big\{X_1=\{2,7,7,8,9\},X_2=\{2,5,7,8,9\}, X_3=\{2,5,7,7,9\}, X_4=\{2,5,7,9,9,\}\, X_5=\{2,7,7,7,9\}, X_6=\{2,7,7,9,9\}, X_7=\{2,6,7,7,9\}, X_8=\{2,6,7,9,9\}\Big\}$.  Let $Y_i$ denote a dataset $X_i$ encrypted under a \nam scheme and $\mathcal{G}^{\mathcal{A}}_{(\alpha,\beta)-\textsf{DI}}(\cdot)$ be the random variable denoting the adversary's output for the $(\alpha,\beta)-\textsf{DI}$ game.  Formally, $(\alpha,\beta)-\textsf{DI}$ is defined as follows.
\\
\textbf{Game} $\mathcal{G}^{\mathcal{A}}_{(\alpha,\beta)-\textsf{DI}}(p)$\begin{enumerate}\item $(X_0,R)\leftarrow \mathcal{A}$ where \begin{enumerate}\item $X_0 \in \mathcal{X}^n, |\mathcal{X}|=N$\item $R=\{i|i\in [n]\}, |R|=\lceil\beta n\rceil $ 
\end{enumerate}\item Construct $Q(X_0)=\{X_1,\cdots,X_q\}$ using Eqs. \eqref{eq:1} and \eqref{eq:2} 
\item Select $p \in \{0,1,\cdots, q\}$ uniformly at random 
\item $p'\leftarrow \mathcal{A}\big(Y_p\big)$ \end{enumerate} 
$\mathcal{A}$ is said to win the above game if $p'=p$.
%Thus, the \textsf{ADR} attack tries to distinguish a that differs in . Moreoevr, each wothn For instance, then advarrsy tries to guess the input dataset after obsrving the output of \nam. recovers the value of any record within $\alpha N$, for a given precision parameter $\alpha \in [1/N,1]$ and recovery rate $\beta \in [0,1]$. Lower the value of $\alpha$, higher is the accuracy in recovering the records. Specifically $\alpha=1/N$ and $\alpha=N$ referring to the cases of exact (adversary correctly identifies all the records) and no database reconstruction (adversary cannot approximate at all), respectively. 
\\\\
\textbf{\cdp Guarantee.} First, we discuss the implications of the \cdp guarantee. Note that $\mathcal{G}^{\mathcal{A}}_{(\alpha,\beta)-\textsf{DI}}(p)=p$ denotes the event that an adversary wins the above game.
 Let $rand$ be a random variable indicating the output of the baseline strategy  where the adversary just performs random guessing.
\begin{theorem}For a \nam scheme satisfying $\epsilon$-\cdp guarantee
\begin{gather}\big|\mathrm{Pr}\big[\mathcal{G}^{\mathcal{A}}_{(\alpha,\beta)-\textsf{DI}}(p)=p \big]-\mathrm{Pr}\big[rand=p\big]\big|\leq \frac{e^{\beta\epsilon^*}}{q+e^{\beta\epsilon^*}}-\Big(\frac{1}{q+1}\Big)^\beta \label{eq:attack:cdp}\end{gather} where $\epsilon^*=\epsilon\cdot\lceil\alpha N\rceil$ and $q=|Q(X_0)|$ (see Step $(2)$ of the  $(\alpha,\beta)-\textsf{DI}$ game). \label{thm:attack:cdp}\end{theorem}
Consider the case when $\lceil\beta n\rceil=1$, i.e., $X_0$ and $X_i \in Q(X_0)$ differ only in a single data point.  In this case,  observe that for low values of $\epsilon^{*}$ (i.e., low $\epsilon$ and $\alpha$) the R.H.S of the Eq. \eqref{eq:attack:cdp} is low. This means that for reasonably low values of $\epsilon$ (high privacy), with very high probability an adversary \textit{cannot distinguish among encrypted datasets that differ in a single point with values reasonably close to each other (small $\alpha$) any better than just random guessing}. In other words, this guarantee rigorously limits the accuracy  of inferencing the value of an individual data point of a dataset. As the value of $\beta$ increases (datasets differ in more than one data point), the protection afforded degrades gracefully. The proof of the above theorem follows directly from the \cdp guarantee and is presented in App. \ref{app:attack}. Note that the above result can take advantage of the privacy amplification by shuffling to provide better protection\footnote{The additional $\delta$ parameter appears as an additive $q\delta$ in Eq. \eqref{eq:attack:cdp}, see App. \ref{app:attack}}. 
 \\\\
 \textbf{\ddp Guarantee.} Next, we focus on the implications of the \ddp guarantee. For this, first we consider a similar indistingushbaility game as before but for a single data point (or record) -- the record indistinguishability attack $\alpha$-\textsf{RI}. Here, the adversary has to distinguish between a single data point $x$ and set of input values $Q(x)$ that differ from $x$ by at most $\lceil\alpha N\rceil$. Let $y_i$ denote the ciphertext for $x_i$ after encryption under \nam and $\mathcal{G}^{\mathcal{A}}_{\alpha-RI}(\cdot)$ represent the random variable denoting the adversary's output for the game which is defined as follows. \\
 \textbf{Game} $\mathcal{G}^{\mathcal{A}}_{\alpha-RI}(p)$
 \begin{enumerate}\item $x_0\leftarrow \mathcal{A}$
 \item $Q(x)=\{x_1, \cdots, x_q\}$ where $x_i \in \mathcal{X}, i \in [q]$ s.t. $|x_0-x_i|\leq \lceil \alpha N\rceil$ and $x_i\neq x_0$  \item Select $p \in \{0,1,\cdots, q\}$ uniformly at random 
\item $p'\leftarrow \mathcal{A}\big(Y_p\big)$ \end{enumerate} 
$\mathcal{A}$ is said to win the above game if $p'=p$.\end{enumerate}

\begin{theorem} 
For a \nam scheme satisfying, we have  \begin{gather}\Big|\mathrm{Pr}[\mathcal{G}^{\mathcal{A}}_{\alpha-RI}(p)=p]-\mathrm{Pr}[rand=p]\Big|\leq \frac{e^{\epsilon^{*}}}{q+e^{\epsilon^{*}}}-\frac{1}{q+1} \label{Eq:attack}\end{gather} where $\epsilon^*=\epsilon\cdot \lceil\alpha N\rceil$.\label{thm:attack:record}
\end{theorem}
From the above theorem,  we observe that \textit{for reasonably low values of $\epsilon$ (high privacy), with very high probability an adversary cannot distinguish among input values that are close to each other (small $\alpha$) any better than just random guessing}. Now, recall that owing to the \ddp guarantee of the underlying \name primitive, every data point encrypted under \nam is also protected by the \ddp guarantee (Lemma \ref{lem:ddp}). 
This means that, for any dataset $X$, the above indistinguishability result holds for every individual data point (record) simultaneously. In other words, \textit{the \ddp guarantee rigorously limits the accuracy of any inference attack for every record of a dataset}. The proof follows directly from the \ddp guarantee and is presented in App. \ref{app:attack}. \par 
As a concrete example, let us look at the binomial attack  on \OPE schemes satisfying \indfaocpa proposed by Grubbs et al. \cite{Grubbs1}. The attack uses a biased coin model to locate the range of ciphertexts corresponding to a particular plaintext. Experimental results on a dataset of first names show that the attack can recover records corresponding to certain high frequency plaintexts (such as first name `Michael') with high accuracy. In this context, the implications of the above result is as follows. Consider a dataset with plaintext records corresponding to first names `Michael' and `Michele'.  For \nam, the recovery rate for either would not be better than the random guessing baseline since both the values are close to each other in alphabetic order. %an adversary cannot distinguish between the twoLet the input domain be just four names $\{'Michael','Michele', 'David','Danny'\}$. On observing the ciphertext corresponding , the adversary can distinguish between records with plaintext values . However, it cannot  If the plaintext of a record is 'Michael', the attack can only that valuethen However, David but cannot say Michael or  Michele (considering for order). 

Next, we present for a result for the aforementioned $(\alpha,\beta)$-\textsf{DI} game for datasets. 
\begin{theorem}For a \nam scheme satisfying $\epsilon$-\ddp guarantee
\begin{gather}\big|\mathrm{Pr}\big[\mathcal{G}^{\mathcal{A}}_{(\alpha,\beta)-\textsf{DI}}(p)=p \big]-\mathrm{Pr}\big[rand=p\big]\big|\leq \Big(\frac{e^{\epsilon^*}}{q+e^{\epsilon^*}}\Big)^\beta-\Big(\frac{1}{q+1}\Big)^\beta \label{eq:attack:ddp}\end{gather} where $\epsilon^*=\epsilon\cdot\lceil\alpha N\rceil$. \label{thm:attack:ddp} \end{theorem} 
Comparing Eqs. \eqref{eq:attack:ddp} and \eqref{eq:attack:cdp} we see that for $\beta > \frac{1}{n}$ and the same value of the privacy parameter $\epsilon$, \ddp gives better protection than \cdp. The proof of the above theorem follows directly from Thm. \ref{thm:attack:record} and is presented in App. \ref{app:attack}.  


Note that all of the presented indistinguishbility results are information-theoretic ones and hold for any adversary --  active or passive, both in the persistent or snapshot attack model \cite{sok}, and regardless of available auxiliary knowledge or input data distribution \cite{sok:DP}.  
\begin{tcolorbox}\textbf{Remark 4.} In the very least, \name scheme \textit{rigorously limits the accuracy of any inference attack for each record of a dataset for all adversaries.} (Thm. \ref{thm:attack:record}). %For the same value of the privacy parameter $\epsilon$, \ddp gives better protection than \cdp (Thm. \ref{thm:attack:cdp}, Thm. \ref{thm:attack:ddp}). However, the \cdp privacy guarantee can be amplified via shuffling (Thm. \ref{thm:amplify:1}).
\end{tcolorbox}



\begin{comment}From the above theorem, observe that for low values of $\epsilon^{*}$ (i.e., low $\epsilon$ and $\alpha$) the R.H.S of the Eq. \ref{Eq:attack} is low. This means that for reasonably low values of $\epsilon$ (high privacy), with very high probability an adversary \textit{cannot retrieve the value of any record of the encrypted database with high accuracy} (small $\alpha$) any better than just random guessing.  %For instance for $N=120$ and $\epsilon=0.05$(\ddp), an adversary cannot approximate any record of the dataset advantage of  over that of random guessing is only of the order of $10^{-5}$. Our expetimental resulst show that, this (SPARC dataset) we achieve good utility under .   
The proof of the above theorem is presented in App \ref{app:thm:attack}. It follows directly from the \ddp guarantee of \nam schemes (Lemma \ref{lem:ddp}) which intuitively prevents any adversary from distinguishing between a pair of input values are close to each. Hence, this clearly disallows high accuracy approximations of the records.

Thus, we obsreve that at the granularity for all the records
Stress on  Regardless of the adversary;s auxiliary kowledge anf onformation theoretic result and holds true for irregardless 
%Note that previous work has outlined several algorithms with varying degrees of efficiency for carrying out the $\alpha$-\textsf{ADR} attack. However, the above theorem is an impossibility result for the attack itself irrespective of the efficiency of the attack algorithm.

  However, if we consider just the \ddp guarantee, then we can assure something at the granularity of each record. For this first consider the following generic attack on. 
 
 This persistent, / active/passive with uxiliray information . 
 \begin{tcolorbox}If a name primitive satisfies $\epsilon_l=\epsilon/2$, then the subsequent )(Lemma T). Additionally, it also satisfies and finally hen, the and the . Now For given by and the subsequent is \end{tcolorbox}
 Reiterating, the relationships between 
 For the vanilla case, 
 
 Extends the guarantee to every single record  simultaneously. This rigorously .
 
 Thus, if the . Thus, States that an adversary
 
 The \textit{persistent access attack} model considers a \textit{persistent} adversary who can observe the database over time. Such an adversary could have knowledge of the individual queries and learn which records are returned in response to each query, i.e, access pattern leakage \cite{generic}. Encrypted database systems employing \OPE are known to be vulnerable to such access pattern leakage \cite{generic} and consequently, to database reconstruction attacks which can recover good approximations of the records of the 
database \cite{Paterson1,Grubbs3,generic}. 
Next, we present an impossibility result for the aforementioned $\alpha$-\textsf{ADR} attack for \nam schemes. Specifically, we show that, with very high probability, an adversary cannot recover the value of even a single record. 
 In order to further demonstrate 
 In order to further the intuitive understanding we present and on a real-world dataset. 
 M%ost of the inference attacks are inherent to any \OPE scheme -- they do not leverage any weakness in the cryptographic security guarantee of the schemes but instead utilize the ordering information of the plaintexts which is revealed as per the definitional requirements of the scheme. In other words, these attacks are beyond the scope of the standard cryptographic security guarantees (like \textsf{IND-FA-OCPA}) for \OPEs and hence, their effects are not captured directly by the cryptographic security guarantees. 
 
 
 \end{comment}
 \subsection{Additional Analysis} In this section, we present additional analysis to further our intuitive understanding of \nam's improved protection against inference attacks. For this, we present a formal model to systematically study the effect of such attacks. We focus on the ``snapshot" attack model (the adversary only obtains a onetime copy or snapshot of the encrypted data store \cite{sok}) for the ease of exposition. The proposed formal model creates a privacy leakage profile for the plaintext bits based on the revealed ordering information and adversary's auxiliary knowledge.
 \\\
\textbf{Model Description.}
 We assume the input domain to be discrete, and finite and w.l.o.g denote it as $\mathcal{X}=[0,2^{m-1}]$. Additionally, let $\mathcal{D}$ represent the true input distribution and $X=\{x_1,\cdots,x_n\}$ be a dataset of size $n$ with each data point sampled i.i.d from $\mathcal{D}$. We model our adversary, $\advppt$, to have access to the following data:
\squishlistnum\item Auxiliary knowledge about a distribution, $\mathcal{D}'$, over the input domain, $\mathcal{X}$. In practice, this can be derived from domain knowledge or auxiliary (public) datasets the adversary has access to. \item The  ciphertexts, $\mathcal{C}$, corresponding to $X$ which represent the snapshot of the encrypted data store.
\squishendnum
The adversary's goal is to recover as many bits of the plaintexts as possible.
Let $X(i), i \in [n]$ represent the plaintext in $X$ with rank~\cite{rank} $i$  and let $X(i,j), j \in [m] $ represent the $j$-th bit for $X(i)$. Additionally, let $b(i,j)$ represent the adversary's guess for $X(i,j)$. Let $\mathcal{L}$ be a $n\times m$ matrix where $\mathcal{L}(i,j)=\mathrm{Pr}\Big[X(i,j)=b(i,j)\big|\mathcal{D},\mathcal{D}'\Big]$ represent the probability that  $\advppt$ correctly identifies the $j$-th bit of the plaintext with rank $i$.
Hence, the matrix $\mathcal{L}$ helps us in analyzing the bitwise information leakage from $\mathcal{C}$ to  $\advppt$.
\begin{comment}Thus $P$ provides a privacy leakage matrix. There can be multiple ways to interpret this matrix, we list a few intersting ones as follows \begin{enumerate}\item Studying the bits with the highest leakage profiles.  \item Studying the \% of bits with leakage probability at most $1/2+\delta$.
\item Studying how many LSB bits with leakage probability at most $1/2+\delta$. \item Studying how many MSB bits with leakage probability at most $1/2+\delta$.  
\end{enumerate}
\end{comment}
\\\textbf{Adversary's Approach.}  $\advppt$'s goal is to produce their best guess for every $X(i,j)$. Hence, given $\advppt$'s auxiliary knowledge about the distribution, $\mathcal{D}'$, the strategy  with   the least probabilistic error is as follows: \begin{gather*} b(i,j)=\arg \max_{b\in \{0,1\}}\{\mathrm{Pr}_{\mathcal{D}'}\big[X(i,j)=b\big]\}, i\in[n], j\in[m]\\= \left\{
                \begin{array}{ll}
                  0 \mbox{ if } \mathbb{E}_{\mathcal{D}'}\big[X(i,j)\big]\leq 1/2\\
                  1 \mbox{ if } \mathbb{E}_{\mathcal{D}'}\big[X(i,j)\big]>1/2
                \end{array}
              \right. \numberthis \label{eq:bit}\end{gather*} 
%Thus, the probability that the adversary succeeds in correctly guessing $x_j[i]$ is \begin{gather}P_{i,j}=Pr\Big[x_j[i]==(x_j[i]')\big|\mathcal{D}\Big]\label{eq:adv}\end{gather}
Next, we compute $\mathcal{L}$ when is $X$ is encrypted under an \OPE scheme that satisfies the \indfaocpa~ security guarantee. This analysis formalizes what  $\advppt$ can learn from just the order of the plaintexts (that is leaked by $\mathcal{C}$ by definition). 
\begin{theorem} If $X$ is encrypted under an \OPE scheme that satisfies the \indfaocpa guarantee, then  for all $i\in [n], j\in [m]$ we have \begin{gather*}\hspace{-1.8cm}\mathcal{L}(i,j)=\sum_{ s \in \mathcal{S}^{j}_{b(i,j)}}\mathrm{Pr}_{\mathcal{D}}\big[X(i)=s\big] \end{gather*}   where $x\sim \mathcal{D}$,  and  $\mathcal{S}^j_{b}=\{s| s \in \mathcal{X} \mbox{ and its }j \mbox{-th bit } s^j=b\}$.\label{thm:formal:OPE}\end{theorem}
 
The bitwise leakage matrix, $\mathcal{L}$, for the case when $X$ is encrypted under a \nam scheme is given as follows.

%Let $j_s$ and $j_e$ denote ranks such that the plaintext corresponding to all the intermediate ranks  $j_s \leq j \leq j_e$ are mapped to the same cipher $c$. Pr[]Thus if for $j \in [j_s,j_e]$,  adversary's guess for the $i$-th bit $x_j[i]'$ is '1', then his/her new expected success probability is, $\mathbb{E}[P_{i,j}]=\sum_{\mathbf{j}\in [j_s,j_e]}\frac{1}{j_e-j_s+1}\cdot \mathbb{P}_{i,\mathbf{j}}$ where $\mathbb{P}_{i,\mathbf{j}}=P_{i,\mathbf{j}}$ if the adversary's guess was $x_\mathbf{j}[i]'=1$, else $\mathbb{P}_{i,\mathbf{j}}=1-P_{i,\mathbf{j}}$. This means that if the adversary prediction for the bits $\{x_j[i]\}, j \in [j_s,j_e]$ are a mix of both $0$s and $1$s, then due to RPOPEc, adversary's attack success rate suffers.

\begin{theorem} If $X$ is encrypted under a \nam scheme, then for all $i\in [n], j\in [m]$ we have \begin{gather*}\mathcal{L}(i,j)=\sum_{s \in S_{b(i,j)}^{j}}\mathrm{Pr}_{\mathcal{D}}\big[x=s\big]\Big(\sum_{v \in \mathcal{O}} \mathrm{Pr}_{\mathcal{D}^*}\big[\widetilde{O}(i)=v\big]\cdot
\\ \hspace{1.5cm}\mathrm{Pr}\big[\name(s,\Pa,\epsilon)=v\big]/\mathrm{Pr}_{\mathcal{D}^*}\big[o=v\big]\ \Big)\end{gather*} where $\widetilde{O}(r)$ denotes the encoding with rank $r, r \in [n]$, $\Pa \in \hat{\mathcal{X}}, o \sim \mathcal{D}^*$, and $\mathcal{D}^*:\mathcal{X}\mapsto\mathcal{O}$ represents the distribution of the encoding $\name(x,\Pa,\epsilon),~x\sim\mathcal{D}$ which is given as \begin{gather*}\mathrm{Pr}_{\mathcal{D}^*}\big[v\big]=\sum_{x\in\mathcal{X}}\mathrm{Pr}_{\mathcal{D}}\big[x\big]\cdot 
\mathrm{Pr}\big[\name(x,\Pa,\epsilon)=v
\big], v\in \mathcal{O}\end{gather*} \label{thm:formal:POPE}\vspace{-0.3cm} \end{theorem}
The proof of the above theorems are presented in App. \ref{app:thm:fm:OPE}. \\ In order to illustrate \nam's gain in protection, we numerically evaluate $\mathcal{L}$ for both a \OPE scheme and a \nam scheme on real world datasets in Fig. \ref{fig:formalmodel:L2:2}.  For this, we use the data from the \textsf{Population} dataset (details in Sec. \ref{sec:evaluation}) for the year $2019$ as the true input distribution, $\mathcal{D}$, and  the data from the year $2011$ is considered to be the adversary's auxiliary distribution, $\mathcal{D}'$. We consider the dataset size to be $200$ and the number of bits considered is $7$ (domain of age is $[1,100]$). Additionally, the partition $\Pa$ for the \name primitive is set to be $\Pa=\mathcal{O}=\mathcal{X}=[1,100]$. The reported privacy parameter $\epsilon$ refers to the $\epsilon$-\indfaocpa guarantee, and implies $\frac{\epsilon}{2}$-\cdp and $\frac{\epsilon}{2}$-\ddp (we do not use privacy amplification here) for the \nam scheme.  As shown in Fig. \ref{fig:formalmodel}, we observe that the probability of successfully recovering the plaintext bits is significantly lower for  \nam as compared to that of a \OPE scheme. Moreover, the probability of recovering the lower-order bits (bits in the right half) is lower than that of  higher-order bits -- the probability of recovering the low-order bits is $\approx 0.5$ which is the random guessing baseline. Recall that Thm. \ref{thm:attack:record} implies that the adversary would not be able to distinguish between pairs of inputs that are close to each other. Hence, the above observation is expected since values that are close to each other are most likely to differ only in the lower-order bits.   
%For instance, the attack first attack in the snapshot model for a \OPE scheme by which tries to . what thsi woudl nena that 0.5 whuch mena s as random guessing baseline. Hence, such an attack would be impossible in . 
Additionally, as expected, the probability of the adversary's success decreases with decreasing value of $\epsilon$. For instance, the average probability of success for the adversary for bit $4$ reduces from $0.77$ in the case of \OPEs (Fig. \ref{fig:formalmodel:L1}) to $0.62$ and $0.51$ for $\epsilon=1$ (Fig. \ref{fig:formalmodel:L2:1}) and $\epsilon=0.1$ (Fig. \ref{fig:formalmodel:L2:2}), respectively, for \nam. 

\begin{figure}
  \begin{subfigure}[b]{0.45\linewidth}
    \centering \includegraphics[width=1\linewidth]{Heatmap_L1.pdf}\vspace{-0.2cm}
        \caption{\scalebox{1}{$\mathcal{L}$ for \OPE}}
        \label{fig:formalmodel:L1}\end{subfigure}
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=1\linewidth]{Heatmap_L2_eps1_1.pdf}\vspace{-0.2cm}
        \caption{\scalebox{1}{$\mathcal{L}$ for \nam for $\epsilon=1$}}
        \label{fig:formalmodel:L2:1}
        \end{subfigure}\\\centering
        \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=1\linewidth]{Heatmap_L2_1.pdf}\vspace{-0.2cm}
        \caption{\scalebox{1}{$\mathcal{L}$ for \nam for $\epsilon=0.1$}}
        \label{fig:formalmodel:L2:2}
        \end{subfigure}
        %\\ \begin{subfigure}[b]{0.45\linewidth}\includegraphics[width=1\linewidth]{Heatmap_L2p.pdf}\caption{$\mathcal{L}$ for \nam for $\epsilon=0.1$}\label{fig:formalmodel:L2p}\end{subfigure}
  
        \caption{Numerical Analysis of the Bitwise Leakage Matrix, $\mathcal{L}$} \label{fig:formalmodel} 
    \end{figure}      %\vspace{-3mm}
     %Note that the aforementioned assumption of an adversary with a prior is made only to capture a real-world instantiation of inference attacks on \OPEs. This assumption has no bearing whatsoever on our primary security guarantee of \indfaocpae~ (Defn. \ref{def:indfaocpae}). 
    %\subsection{Persistent Access Attack Model} 



















\begin{comment}

\begin{gather*}\mathrm{Pr}[x_j[i]==1]=\sum_{k=1}^m \mathrm{Pr}[B_{i,k}]\cdot \mathrm{Pr}\Big[x_j[i]==1\Big|B_{i,k}\Big]\end{gather*}
Now, \begin{gather*}x \sim \mathcal{D}\\ S_{i,1}=\{y|y \in \{0,\cdots,\mathbb{S}-1\} \wedge y[i]==1\}\\S_{i,0}=\{y|y \in \{0,\cdots,\mathbb{S}-1\} \wedge y[i]==0\}\\Pr[B_{i,k}]={m \choose k}\cdot \big(Pr[x \in S_{i,1}|\mathcal{D})^{k} \cdot \big(Pr[x \in S_{i,0}|\mathcal{D}]\big)^{m-k} \end{gather*}
Let Additionally, we have \begin{gather*}
Pr[x_j[i]==1\Big| B_{i,k}]=\sum_{y \in S_{i,1}} Pr[x_j==y]\cdot Pr[D_{i,k-1}]
\end{gather*}

Now, the order this 
Now if we assume that $\mathcal{D}$ is uniform distribution, i.e., $Pr[x=t]=\frac{1}{\mathbb{S}}, x \sim \mathcal{D}, t \in \{0,\cdots,\mathbb{S}-1\}$, then 
\begin{gather*}Pr_{\mathcal{D}}[x_j==y]=\Big(\frac{y+1}{\mathbb{S}}\Big)^{j-1}\cdot\frac{1}{\mathbb{S}}\cdot\Big(\frac{\mathbb{S}-y}{\mathbb{S}}\Big)^{m-j}\end{gather*}
\textbf{Analysis for} \textsf{IND-FA-OCPA}:
Recall the  Specifically, without loss of generality, we consider that the plaintext domain is $\{0,\cdots,\mathbb{S}-1\}$. (As long as, the original plaintext domain size is $\mathbb{S}$, we can re-map the plaintexts to be in the domain $\{0,\cdots,\mathbb{S}-1\}$.) Again for the ease of analysis we consider $\mathbb{S}=2^s$.  essentially means analyzing what can be learnt just from the order of $\{x_i\}$, i.e., assume $\mathcal{A}$ has access to a set of $m$ ciphers corresponding to an OPE scheme with IND-FAOCPA guarantee \cite{IND-FA-OCPA}.  


\subsubsection{Adversary Auxiliary Knowledge}
Recall that we assume the adversary $\mathcal{A}$ has auxiliary knowledge about a distribution $\mathcal{D}'$ such that $||\mathcal{D}-\mathcal{D}||_1\geq \delta$. This can be modeled in different ways. We list few interesting ones as follows
\begin{itemize}\item If the distribution is parametric (Binomial distribution) and the adversary has an estimate of the parameters with error $O(f(\delta))$.\item  Assume that the auxiliary distribution known to the adversary differs in only a small number (like 2) of domain (plaintext) items, i.e., $\mathcal{D}'(i)=\mathcal{D}(i) \forall i \in domain(\mathcal{D})/ \{j,k\}, \mathcal{D}'(j)=\mathcal{D}(j)+\frac{\delta}{2},\mathcal{D}'(k)=\mathcal{D}(k)-\frac{\delta}{2}$.  \item 
Assume that the adversary has a good estimation about some $t$ fraction of the values in the domain, $S_t$, and uses uniform distribution for the rest of the numbers such that $\sum_{l\in S_t}|\mathcal{D}[l]-\mathcal{D}'[l]|\approx \delta', \delta'<<\delta, \delta'+ \sum_{l \in domain(\mathcal{D})/S_t} |\mathcal{D}[l]-\frac{1-\sum_{l\in S_t}\mathcal{D}'[l]}{|domain(\mathcal{D})|-|S_t|}|\geq \delta$ \item For each number $l$ in the domain, $|\mathcal{D}[l]-\mathcal{D}'[l]|\geq \delta_l, \sum_l \delta_l \geq \delta$.\end{itemize}
It would be interesting to analyse the $P_{ij}, j \in [m], i \in [n]$ for each of the above cases. \arc{TODO} %and find the corresponding RPOPEc parameters $\rho_l, l \in [r]$ such that it minimizes $P_{ij}$ at a chosen level of utility.
\end{comment}

\begin{comment}Let bit $b=x_j[i]'$, i.e., the guess of the adversary $\mathcal{A}$ for the bit $x_j[i]$. Let $S_{i,b}=\{y|y \in \{0,\cdots,\mathbb{S}-1\} \wedge y[i]==b\}$. Then, assuming $\mathcal{M}$ is the RPOPEc mechanism we have
\small{\begin{gather}E[P_{ij}]=\sum_{e \in [j,n]}\Bigg(\sum_{s \in [1,j]}\frac{1}{j-s+1}\sum_{c\in [r]}\Big(\prod_{k \in [s,e]}(\sum_{y \in S_{i,b}}Pr_{\mathcal{D}}[x_k[i]==y]\cdot Pr[\mathcal{M}(y)==c]\big)\Big)\Bigg) \label{eq:adversary}\end{gather}}
\end{comment}



%\begin{tcolorbox} \textbf{Remark 3.} In the very least,  \nam schemes rigorously limits the approximation accuracy of every record for any adversary (even under inference attacks, Thm. \ref{thm:attack}). For agiven value that However, the privacy paramer can be amplied via shuffling (). %Every record of a database encrypted under a \nam scheme satisfies \ddp which prevents any adversary from distinguishing between a pair of input values are close to each. This means that, in the very least, the lower order bits of all records are protected even in the face of inferential attacks (both in the snapshot and persistent adversary attack models). 
%\end{tcolorbox}
%Note that the security guarantee of the \nam scheme only relies on the $\epsilon$-\ddp guarantee from the underlying \name primitive. In other words, the choice of the partition does not . This is so beacuse regardless of the  it is completely agnostic of the choice of partition   - the partition only affects the utility via the overhead as explained above. does not utilise the on the choice of the partition - it just . As explained in The partition is just from an utilitarian perspective, the which is $\epsilon$ is independent of the 

==> protocol2.tex <==
\section{Proposed Primitives} \label{sec:protocol}
In this section, we discuss our proposed primitives. First, we introduce our $\epsilon$-\ddp \textit{%partially 
order preserving encoding scheme}, \name. %which allows under $\epsilon$-\ddp guarantee. 
Next, we describe our $\epsilon$-\ddp \textit{%partially 
order preserving encryption scheme} (\nam)  that is based on  the \name primitive.
\subsection{$\epsilon$-\ddp %Partially 
Order Preserving Encoding (\name)}\label{sec:encoding}
\name is a randomised mechanism that encodes its input while maintaining some of its ordinal characteristics. If $\mathcal{X}=[s,e]$ is an input domain, then a $k$-partition $\mathcal{P}$ on $\mathcal{X}$ denotes a set of $k$ non-overlapping intervals $\mathcal{X}_i=(s_i,e_i]$
\footnote{The first interval $\mathcal{X}_1=[s,e_1]$ is a closed interval.}, $s_{j+1}=e_j, i \in [k], j \in [k-1]$ such that $\bigcup_{i=1}^k \mathcal{X}_i=\mathcal{X}$. For example, for an input domain $\mathcal{X}=[1,100]$, $\Pa=\{[1,10],(10,20],\cdots,(90,100]\}$ denotes a $10$-partition. Let $\hat{\mathcal{X}}$ denote the domain of partitions defined over $\mathcal{X}$. For brevity, we denote a partition as a set of the end points $e_i$ for each of its intervals. For instance, from the above example,  $\Pa=\{10,20,\cdots,90,100\}$. Additionally, let $\mathcal{O}=\{o_1, \cdots, o_k\}, o_i<o_{i+1}, i \in [k-1]$ represent the output domain where $o_i$ is the corresponding encoding for the interval $\mathcal{X}_i$ and let $\mathcal{P}(x)=o_i$ denote that $x \in \mathcal{X}_i$. Referring back to our example, if $\mathcal{O}=\{1,2,\cdots,10\}$, then  $\Pa(45)=5$.

\begin{definition}[$\epsilon$-\ddp %Partially 
Order Preserving Encoding] A \textit{$\epsilon$-\ddp %partially 
order preserving encoding} scheme, $\name:\mathcal{X}\times\hat{\mathcal{X}} \times \mathbb{R}_{>0}\mapsto \mathcal{O}$ is a randomized mechanism such that 
\begin{enumerate} \item $|\mathcal{O}| = k$ \item For all $ x \in \mathcal{X}, o \in \mathcal{O}/\mathcal{P}(x)$ we have \begin{gather*}\hspace{-4cm}\mathrm{Pr}\big[\name(x,\Pa,\epsilon)= \mathcal{P}(x)\big]> \\\hspace{2.8cm}\mathrm{Pr}\big[\name(x,\Pa,\epsilon)= o\big]\numberthis\label{eq:popec:order}\end{gather*} 
\item For all $x,x' \in \mathcal{X}, o \in \mathcal{O}$ such that $|x-x'|\leq t$, we have \begin{gather*} 
\hspace{-4cm}\mathrm{Pr}\big[\name(x,\Pa,\epsilon)=o\big]\leq\\ \hspace{2cm}e^{t\epsilon}\cdot \mathrm{Pr}\big[\name(x',\Pa,\epsilon)=o\big]\numberthis\label{eq:popec:dp}\end{gather*} \end{enumerate}
where $\Pa\in \hat{\mathcal{X}}$ is a $k$-partition. \label{def:popec}
\end{definition} 

The first property in the above definition signifies the flexibility of the \name primitive to provide only a \textit{partial} ordering guarantee. For instance, in our above example $k=10 < |\mathcal{X}|=100$. $\Pa=\mathcal{O}=\mathcal{X}$ denotes the default case where effectively no partition is defined on the input domain and  $\Pa(x)=x, x \in \mathcal{X}$ trivially. Note that, due to randomization (required due to the \ddp guarantee), \name is bound to incur some errors in the resulting numerical ordering of its outputs. To this end, the second property guarantees that the noisy output is most likely to be the correct one. For instance, $\Pa(45)=5$ is the most likely output for $\name(45,\Pa,\epsilon)$.  This ensures that the noisy outputs still retain sufficient ordinal characteristics of the corresponding inputs. 
 The second property ensures that the primitive satisfies $\epsilon$-\ddp. Note that, $\epsilon=\infty$ represents the trivial case $\name(X,\Pa,\infty)=\Pa(X)$.

\input{construction_copu}
\subsection{$\epsilon$-\cdp %Partially 
Order Preserving Encryption (\nam)}\label{sec:encryption}
As discussed in Sec. \ref{sec:intro}, the \textit{$\epsilon$-\cdp %partially
order preserving  encryption} (\nam) scheme is an encryption scheme that bolsters the cryptographic guarantee of a \OPE scheme with an additional \cdp guarantee. 
Here, we detail how our proposed primitive \name can be used in conjunction with a \OPE scheme (Defn. \ref{def:OPE}) to form a \nam scheme. 
%Let $\mathcal{E}=\langle \textsf{K}, \textsf{E}, \textsf{D} \rangle$ be a \OPE scheme that satisfies $\textsf{IND-FA-OCPA}$ guarantee and $\s\leftarrow \textsf{K}(1^\kappa)$ be the secret key (or state) where $\kappa$ is the security parameter. Let $x$ denote an input data point for the encryption scheme. 
\begin{definition}[$\epsilon$-\cdp %Partially 
Order Preserving Encryption] A \textit{$\epsilon$-\cdp %partially 
order preserving encryption} scheme, \nam, is composed of a \OPE scheme, $\mathcal{E}$ that satisfies the $\indfaocpa$ guarantee, and \name and is defined by the follow three algorithms: 
\begin{itemize}
\item \textit{Key Generation} ($\textsf{K}_{\epsilon}$). Uses $\K$ from the \OPE scheme to generate a secret key $\s$.
\item \textit{Encryption} ($\textsf{E}_{\epsilon}$). The encryption algorithm inputs data sequence $X \in \mathcal{X}^n$, an  order $\Gamma$, a partition $\Pa \in \hat{\mathcal{X}}$, and the privacy parameter $\epsilon$. The encryption works as follows:
\begin{enumerate} %\item For the first point $x_1$, apply the proposed randomised \name~ to obtain $\name(x_1)$. Next, encrypt to obtain the final ciphers $\textsf{E}(\name(x_1),k,\Gamma_1)$. 
\item Set $\s_0\leftarrow\K(\kappa)$
\item For $\forall i \in [n]$, compute $(\s_{i},y_i)\leftarrow \E(\s_{i-1}, o_i,\Gamma,i)$ where $o_i\leftarrow\name(x_i,\Pa,\epsilon/2)$\end{enumerate}
\item \textit{Decryption} ($\D_\epsilon$). The decryption algorithm uses \textsf{D} to get back $o_i\leftarrow \D(\s_{i-1},y_i)$.
\end{itemize}\label{def:pope}
\end{definition}
\textbf{Key Idea.} The key idea of the above definition is that the \OPE scheme is applied to the output of the \name primitive. Thus, ciphertexts encrypted under \nam preserve the order of the corresponding encodings as output by the \name primitive. Referring back to our example, if $X=\{76,9,9,40,15,76,77\}$ and its corresponding encodings are $O=\{8,1,2,4,2,8,8,8\}$, then the encryption of $X$ under \nam preserves the order of $O$. \par In other words, since a \OPE scheme preserves the exact order of its input data sequence by definition, the utility of \nam (in terms of the preserved ordering information) is determined by the underlying \name primitive. This is formalized by the following theorem.
%An \OPE scheme preserves the exact ordering of the plaintexts. However, the \nam scheme incurs a loss of some of the ordering information due to the error from the randomization (pre-requisite for the \DP guarantee). Additionally, we only obtain a partial ordering of the ciphertexts, i.e., there exists some pairs of data points (encrypted under \nam) that are incomparable.
%Specifically, the values that fall in the same interval in the partition $\mathcal{P}$, i.e., the values that are close to each other are most likely to be incomparable. 
\begin{theorem}[Utility Theorem] If, for a given partition $\Pa\in \hat{\mathcal{X}}$  and for all $x,x' \in \mathcal{X}$ such that $x > x'$ we have \begin{gather}\mathrm{Pr}\big[\name(x,\Pa,\epsilon)\geq \name(x',\Pa,\epsilon)\big]\geq \alpha\end{gather} for $ \alpha \in [0,1]$, then for a \nam scheme instantiated on such a \name, we have
 \begin{gather}\mathrm{Pr}\big[\E_{\epsilon}(x,\s,\Gamma,\Pa,\epsilon)\geq \E_{\epsilon}(x',\s,\Gamma,\Pa,\epsilon) \big]\geq \alpha\end{gather} where $\s\leftarrow \K_{\epsilon}(\kappa)$  and $\Gamma=\{1\}$ trivially. \end{theorem} 
 The proof of the above theorem follows directly from Defns. \ref{def:OPE} and \ref{def:pope}.
\begin{comment}\begin{proof} ote that, hence this is for ideal world where . Now n P()*P()
Frequency that each of them \begin{gather*}\mathrm{Pr}[P(x_i)>y]=\sum_{c}Pr[]\cdot Pr[\leq c]\\=\sum_c
Pr[\name(x)=c]\cdot (\sum_{c'<c}) Pr[\name(y)=c']\\\geq Pr[\name(x)=c_i]/e^{d\cdot \epsilon}\end{gather*} \end{proof}
number of 
Number of mismatch
\begin{gather*}\sum_{i=0}^k{ n \choose i }\alpha^{n-i}\cdot (1-\alpha)^i \\=\alpha^{n}\frac{\Big(\frac{(n-k)\cdot (1-\alpha)}{k\cdot\alpha}\Big)^k-1)}{\frac{n-k}{k\cdot \alpha}-1}\end{gather*}
|Partition 
\end{comment}
%We are that the order information is laced with a layer of DP guarantee. 






